Non-invasive in silico determination of ventricular wall pre-straining and characteristic cavity pressures

The clinical application of patient-specific modelling of the heart can provide valuable insights in supplementing and advancing methods of diagnosis as well as helping to devise the best possible therapeutic approach for each individual pathological heart condition. The potential of computational cardiac mechanics, however, has not yet been fully leveraged due to the heart's complex physiology and limitations in the non-invasive in vivo characterisation of heart properties necessary required for accurate patient-specific modelling such as the heart anatomy in an unloaded state, ventricular pressure, the elastic constitutive parameters and the myocardial muscle fibre orientation distribution. From a solid mechanics point of view without prior knowledge of the unloaded heart configuration and the cavity pressure-volume evolution, in particular, the constitutive parameters cannot be accurately estimated to describe the highly nonlinear elastic material behaviour of myocardial tissue. Here, knowledge of the volume-normalized end-diastolic pressure relation for larger mammals is exploited in combination with a novel iterative inverse parameter optimisation framework to determine end-systolic and end diastolic pressures, ventricular wall pre-straining and pre-stressing due the residual end-systolic cavity pressure as well as myocardial tissue stiffness parameters for biventricular heart models.

==> package_preamble.tex <==
% -----------------------------------------
% UK language and time format
% -----------------------------------------
\usepackage[UKenglish]{babel}
\usepackage[UKenglish]{isodate}

% -----------------------------------------
% Page manipulation
% -----------------------------------------
\usepackage{lscape}

% -----------------------------------------
% Text manipulation
% -----------------------------------------
\usepackage{lipsum} % to fill in with arbitrary text
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor} % Allows text to be written in different colours
\usepackage[final, babel, protrusion=true,expansion=true]{microtype}
\usepackage[super]{nth}
\usepackage{setspace}

% -----------------------------------------
% Mathematics packages
% -----------------------------------------
\usepackage[fleqn]{mathtools}
\usepackage{amsfonts,amssymb,amsthm,amsbsy}
\usepackage[binary-units=true]{siunitx}
\usepackage{wasysym} % diameter symbol

% -----------------------------------------
% Text fonts
% -----------------------------------------
%\usepackage[sc,osf]{mathpazo} % add possibly `sc` and `osf` options
%\usepackage{eulervm}
%\usepackage{mathptmx}
\usepackage{newtxtext}
\usepackage[varg, cmintegrals, cmbraces]{newtxmath} % has to be placed after amsmath
\usepackage{eufrak}
\usepackage{ulem}

% -----------------------------------------
% Pictures/Images packages/commands
% -----------------------------------------
% Obsolete: sufigure
% Buggy: subfig - Hyperref doesn't work properly 
%\usepackage[tight,footnotesize]{subfigure}
\usepackage{graphicx}
\usepackage{float}
\usepackage{fancybox}
% Draws a frame around picture
\usepackage[export]{adjustbox}
\usepackage[hypcap]{caption}
\usepackage{subcaption} 
\usepackage{epstopdf}

\usepackage{soul}
\newcommand{\hlc}[2][yellow]{ {\sethlcolor{#1} \hl{#2}} }

% -----------------------------------------
% Tables
% -----------------------------------------
\usepackage{booktabs}
\usepackage{multirow}

% -----------------------------------------
% Lists
% -----------------------------------------
\usepackage{enumitem}


% -----------------------------------------
% Bibliography related packages/commands
% -----------------------------------------
% Using the NATBIB referencing environment
%\usepackage[square,sort,numbers]{natbib}
%
% Using the BIBLATEX referencing environment
%\usepackage[backend=biber,natbib=true]{biblatex}
%\usepackage[natbib=true]{biblatex}
%\bibliography{./Reference/MyRef}
%
% Handle cross-referencing
\usepackage[colorlinks=true,allcolors={blue},bookmarks]{hyperref}
%
% Create web-link for every DOI 
%\usepackage{doi}

% -----------------------------------------
% Display algorithms
% -----------------------------------------
%\usepackage{algorithmic}
%\usepackage{algorithm}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\makeatletter
\def\BState{\State\hskip-\ALG@thistlm}
\makeatother
%\newcommand{\INDSTATE}[1][1]{\STATE\hspace{#1\algorithmicindent}}


% -----------------------------------------
% Table manipulation
% -----------------------------------------
\usepackage{multirow}


% -----------------------------------------
% SI Units manipulation
% -----------------------------------------
\usepackage[binary-units=true]{siunitx}


% -----------------------------------------
% TOC related stuff
% -----------------------------------------
% Include Appendix in TOC
\usepackage[titletoc]{appendix}
\usepackage{accents}

% Extend the TOC numbering
\setcounter{secnumdepth}{4}
\setcounter{tocdepth}{4}


% -----------------------------------------
% Nomenclature related stuff
% -----------------------------------------
\usepackage{todonotes}
\usepackage[refeq,refpage]{nomencl}
% command : makeindex thesis.nlo -s nomencl.ist -o thesis.nls
% Line spacing in nomenclature
\setlength{\nomitemsep}{-\parsep}
% Defining section in nomenclature
%\renewcommand{\nomgroup}[1]{%
%\ifthenelse{\equal{#1}{A}}{\item[\textbf{\textit{Symbols}}]}{
%\vspace{0.1cm}
%\ifthenelse{\equal{#1}{B}}{\item[\textbf{\textit{Greek Letters}}]}{}
%\vspace{0.15cm}
%\ifthenelse{\equal{#1}{C}}{\item[\textbf{\textit{Acronyms}}]}{}}}


% -----------------------------------------
% Display line numbers
% -----------------------------------------
\usepackage[switch,right,displaymath,mathlines]{lineno}
%\linenumbers
